Electromagnetic Signatures of Dark Photon Superradiance

Black hole superradiance is a powerful tool in the search for ultra-light bosons. Constraints on the existence of such particles have been derived from the observation of highly spinning black holes, absence of continuous gravitational-wave signals, and of the associated stochastic background. However, these constraints are only strictly speaking valid in the limit where the boson's interactions can be neglected. In this work we investigate the extent to which the superradiant growth of an ultra-light dark photon can be quenched via scattering processes with ambient electrons. For dark photon masses $m_{\gamma^\prime} \gtrsim 10^{-17}\,{\rm eV}$, and for reasonable values of the ambient electron number density, we find superradiance can be quenched prior to extracting a significant fraction of the black-hole spin. For sufficiently large $m_{\gamma^\prime}$ and small electron number densities, the in-medium suppression of the kinetic mixing can be efficiently removed, and quenching occurs for mixings $\chi_0 \gtrsim \mathcal{O}(10^{-8})$; at low masses, however, in-medium effects strongly inhibit otherwise efficient scattering processes from dissipating energy. Intriguingly, this quenching leads to a time- and energy-oscillating electromagnetic signature, with luminosities potentially extending up to $\sim 10^{57}\,{\rm erg / s}$, suggesting that such events should be detectable with existing telescopes. As a byproduct we also show that superradiance cannot be used to constrain a small mass for the Standard Model photon.

==> app.tex <==

\section{Plasma frequency around BHs} \label{app:plasma}

\paolo{Working on this}

In this appendix we estimate the typical plasma density expected in the surrounding of an astrophysical BH. For a plasma with electron density $n_e$, the plasma density reads
%%%
\begin{equation}
 \omega_p=\sqrt{\frac{4\pi n_e e^2}{m_e}}\,.
\end{equation}
%%%


In order to estimate the typical electron density we use a simple Bondi-Hoyle model for spherical accretion onto a BH moving relative to a background baryonic density,
\begin{equation}
	\frac{d M}{dt} = {4\pi \lambda \rho_\infty}{v_{\rm eff}} r_B^2\, ,
\end{equation}
where $\lambda={\cal O}(1)$ is a model-dependent factor that accounts for the non-gravitational suppression of accretion, $\rho_\infty$ is the density far from the BH, and $v_{\rm eff} = \sqrt{c_\infty^2 + v_{\rm rel}^2}$, where $c_\infty$ and $v_{\rm rel}$ are the speed of sound and the relative BH-baryon velocity far from the BH, respectively, and
%%%
\begin{equation}
 r_B = \frac{M}{v_{\rm eff}^2}
\end{equation}
%%%
is the Bondi radius. For typical non-relativistic effective velocities, $r_B\gg M$, so the Bondi radius is much bigger than the BH gravitational radius.
In this regime the total infalling flow of baryons towards the BH is roughly constant, i.e.
\be
n_e(r) v_{\rm ff}(r)r^2 = {\rm const} 
\ee
where $v_{ff}(r)=\sqrt{v^2_{\rm eff}+\frac{2M}{r}-\frac{2M}{r_B}}$ is the free fall velocity of the gas, which reduces to $v_{\rm eff}$ at the Bondi radius. Therefore, the electron density profile within the Bondi sphere reads
%%%
\begin{equation}
 n_e(r) = n_e^{\infty} \frac{v_{\rm eff}r_B^2}{v_{\rm ff}(r) r^2}\,,\label{densityprof}
\end{equation}
%%%
where $n_e^{\infty}=\rho_\infty/m_e$.
%
At distances $r\sim 2M$, $v_{ff}(r)\sim \sqrt{2M/r}\gg v_{\rm eff}$, so that 
%%%
\begin{equation}
 n_e(r) \sim n_e^{\infty} \frac{v_{\rm eff}}{\sqrt{2M}} \frac{r_B^2}{ r^{3/2}}\,,\label{densityprof2}
\end{equation}
%%%
Finally, near the peak of the BH-boson condensate, $r_{\rm cloud}\sim M/\alpha^2$, we get 
%%%
%%%
\begin{equation}
 n_e(r_{\rm cloud}) \sim \frac{n_e^{\infty} }{\sqrt{2}v_{\rm eff}^3} \alpha^3 \approx 10^3 n_e^{\infty} \left(\frac{\alpha}{0.1}\right)^3 \left(\frac{0.01}{v_{\rm eff}}\right)^3\,,\label{densityprofF}
\end{equation}
%%%
which is valid provided $r_{\rm cloud}\lesssim r_B$, i.e. $\alpha\gtrsim v_{\rm eff}$. The above estimate shows that the typical electron density in the relevant region near the BH can be several orders of magnitude larger than the ``ambient'' density at infinity, $n_e^{\infty}$, depending on $\alpha$ and $v_{\rm eff}$. Correspondingly, the plasma density $\omega_p\propto n_e^{1/2}$ can also vary by some orders of magnitude.
%
In the main text we AAA




is computed by assuming that at large distances, $R \sim 
r^\text{\tiny bin}_\text{\tiny B} $, it reduces to the usual effective velocity $v_\text{\tiny eff}$, i.e.
\be
v_\text{\tiny ff} (R) = \sqrt{v^2_\text{\tiny eff} + \frac{2M_\text{\tiny tot}}{R} - \frac{2M_\text{\tiny 
			tot}}{r^\text{\tiny bin}_\text{\tiny B}}}\,,



\paolo{OLD:}


% Let us begin by estimating the minimum electron number density. The Bondi-Hoyle accretion rate for a BH moving relative to a background baryonic density is given by 

Focusing on the volume where the dark photon bound states reside, and converting the differential rate of mass accretion to the average change in electron number density, one can write
\begin{equation}
	\frac{dn_e}{dt} \sim \frac{3\lambda}{8\pi^3} \frac{\alpha^2 m_{\gamma^\prime}}{v_{\rm eff}^3} \, \overline{n}_e (z) \, \Delta_e \, 
\end{equation}
where we have re-written the asymptotic electron density in terms of the cosmological mean average and the electron 
overdensity $\Delta_e$. The value of $n_e$ we adopt for our calculations should be sufficiently large such that it does 
not change over the timescale required to generate the superradiant cloud, which is typically no larger than $10^{3} 
\tau_{sr}$. \paolo{Question} If we now adopt extremal values so as to minimize the accretion rate (specifically, taking 
$\lambda \sim 10^{-2}$, $v_{\rm eff} \sim 10^{-1}$ \footnote{This value is motivated from the maximum `super-kick' that 
may be imparted to BHs generated in binary merges~\cite{Sperhake:2010uv}. While this is not expected to the 
norm, such an extreme value serves the purpose of estimating a lower limit on the accretion rate. }, $\Delta_e \sim 1$, 
and $z \sim 0$), we find that for $\alpha = 0.05$ and $\alpha = 0.4$ the net accretion over a timescale of $10^3 
\tau_{sr}$ is around $10^{-7}$ and $5 \times 10^{-5} \, {\rm cm^{-3}}$. From this estimate, we adopt a threshold for the 
minimal local electron number density of $\sim 10^{-4} \, {\rm cm}^{-3}$. For more realistic values, namely taking 
$v_{\rm eff} \sim 10^{-3}$ and $\Delta_e \sim 10^{3}$, we find for $\alpha = 0.4$ a change in the electron number 
density of slightly larger than $10^{4} \, {\rm cm}^3$. Note that this estimate is roughly consistent with more rigorous 
treatments of the Bondi accretion problem~\cite{johnson2007effects}, and not far off from the inferred values near the 
supermassive BH in the Galactic Center~\cite{wang2013dissecting,rozanska2015x,zajavcek2018charge}. We thus 
choose to adopt a fiducial electron number density for our analysis of $10^{4} \, {\rm cm}^{-3}$, although this value 
may vary by orders of magnitude in either direction. 

\paolo{For the above estimate, we could use an argument similar to eq. 2.17 here: https://arxiv.org/abs/2005.05641}

